Graph Data Augmentation for Graph Machine Learning: A Survey

Data augmentation has recently seen increased interest in graph machine learning given its demonstrated ability to improve model performance and generalization by added training data. Despite this recent surge, the area is still relatively under-explored, due to the challenges brought by complex, non-Euclidean structure of graph data, which limits the direct analogizing of traditional augmentation operations on other types of image, video or text data. Our work aims to give a necessary and timely overview of existing graph data augmentation methods; notably, we present a comprehensive and systematic survey of graph data augmentation approaches, summarizing the literature in a structured manner. We first introduce three different taxonomies for categorizing graph data augmentation methods from the data, task, and learning perspectives, respectively. Next, we introduce recent advances in graph data augmentation, differentiated by their methodologies and applications. We conclude by outlining currently unsolved challenges and directions for future research. Overall, our work aims to clarify the landscape of existing literature in graph data augmentation and motivates additional work in this area, providing a helpful resource for researchers and practitioners in the broader graph machine learning domain. Additionally, we provide a continuously updated reading list at https://github.com/zhao-tong/graph-data-augmentation-papers.

==> 8gda-sl.tex <==

\begin{table*}[t]
% \small
\caption{A summary of graph data augmentation techniques for graph machine learning. Task levels: V: node-level; G: graph-level; E: edge-level. Augmented data categories: V: node; E: edge; X: feature; G: subgraph. \\ $^\dag$Although GRAND and NodeAug are semi-supervised methods, they used GDA operations with only self-supervised learning objectives (i.e, consistency loss). Therefore, we categorize their GDA techniques as designed for self-supervised learning objectives.}
% \vspace{-0.1in}
\label{tab:methods}
\centering
\Scale[1]{\begin{tabular}{l|l|ccc|cccc|l}
\toprule
\multicolumn{2}{c|}{} & \multicolumn{3}{c|}{Task Level} & \multicolumn{4}{c|}{Augmented Data} & \multirow{2}{*}{Augmentation Methodology} \\
\multicolumn{2}{c|}{} & V & G & E & V & E & X & G \\
\midrule
% \parbox[t]{2mm}{\multirow{27}{*}{\rotatebox[origin=c]{90}{GDA for Supervised Objective}}}
% & DropEdge~\cite{rong2019dropedge} & \cmark &  &  &  & \cmark &  &  & \multirow{4}{1in}{Edge dropping} \\
% & NeuralSparse~\cite{zheng2020robust} & \cmark &  &  &  & \cmark &  &  \\
% & TADropEdge~\cite{gao2021training} & \cmark &  &  &  & \cmark &  &  \\
% & FairDrop~\cite{spinelli2021fairdrop} & \cmark &  &  &  & \cmark &  &  \\
% \cmidrule(lr){2-10}
% & GDC~\cite{klicpera2019diffusion} & \cmark &  &  &  & \cmark &  &  & \multirow{2}{1in}{Graph diffusion} \\
% & MV-GCN~\cite{yuan2021semi} & \cmark &  &  &  & \cmark &  &  \\
% \cmidrule(lr){2-10}
% & AdaEdge~\cite{chen2020measuring} & \cmark &  &  &  & \cmark &  &  & \multirow{6}{1in}{Structure prediction} \\
% & Pro-GNN~\cite{jin2020graph} & \cmark &  &  &  & \cmark &  & \\
% & GAug-M~\cite{zhao2021data} & \cmark &  &  &  & \cmark &  &  \\
% & GAug-O~\cite{zhao2021data} & \cmark &  &  &  & \cmark &  &  \\
% & Eland~\cite{zhao2021action} & \cmark &  &  &  & \cmark &  &  \\
% & MH-Aug~\cite{park2021metropolis} & \cmark &  &  &  & \cmark &  &  \\
% \cmidrule(lr){2-10}
% & FLAG~\cite{kong2020flag} & \cmark & \cmark & \cmark &  &  & \cmark & & \multirow{3}{1in}{Feature generation} \\
% & LA-GNN~\cite{liu2021local} & \cmark &  &  &  &  & \cmark &  \\
% & \citet{tang2021data} & \cmark &  &  &  & \cmark & \cmark &  \\
% & SR+DR~\cite{song2021topological} & \cmark &  &  &  &  & \cmark &  \\
% \cmidrule(lr){2-10}
% & AutoGRL~\cite{sun2021automated} & \cmark &  &  & \cmark & \cmark & \cmark &  & AutoML \\
% \cmidrule(lr){2-10}
% & CoGSL~\cite{liu2022compact} & \cmark &  &  &  & \cmark &  &  \\
% \cmidrule(lr){2-10}
% & GraphMix~\cite{verma2019graphmix} & \cmark &  &  & \cmark &  &  &  & \multirow{4}{1in}{Mixup} \\
% & Graph Mixup~\cite{wang2021mixup} & \cmark & \cmark &  & \cmark &  &  & \cmark \\
% & ifMixup~\cite{guo2021intrusion} &  & \cmark &  &  &  &  & \cmark \\
% & Graph Transparent~\cite{park2021graph} &  & \cmark &  &  &  &  & \cmark \\
% \cmidrule(lr){2-10}
% & GraphCrop~\cite{wang2020graphcrop} &  & \cmark &  &  &  &  & \cmark & Subgraph cropping \\
% \cmidrule(lr){2-10}
% & MoCL~\cite{sun2021mocl} &  & \cmark &  &  &  &  & \cmark & Substructure substitution \\
% \cmidrule(lr){2-10}
% & M-Evolve~\cite{zhou2020data} &  & \cmark &  &  & \cmark &  &  & Motif-similarity mapping \\
% \cmidrule(lr){2-10}
% & CFLP~\cite{zhao2021counterfactual} &  &  & \cmark &  & \cmark &  &  & Counterfactual augmentation \\
% \cmidrule(lr){2-10}
% & MeTA~\cite{wang2021adaptive} &  &  & \cmark &  &  &  &  & Edge perturbation \\
% \midrule
\parbox[t]{2mm}{\multirow{16}{*}{\rotatebox[origin=c]{90}{GDA for Self-supervised Objective}}}
& DGI~\cite{velickovic2019deep} & \cmark &  &  &  &  & \cmark &  & \multirow{7}{1in}{Corruption} \\
& GraphCL~\cite{you2020graph} &  & \cmark &  & \cmark & \cmark & \cmark & \cmark \\
& GRACE~\cite{zhu2020deep} & \cmark &  &  &  & \cmark & \cmark &  \\
& SUBG-CON~\cite{jiao2020sub} & \cmark &  &  &  &  &  & \cmark \\
& InfoGCL~\cite{xu2021infogcl} & \cmark &  &  & \cmark & \cmark &  & \cmark \\
& BGRL~\cite{thakoor2022largescale} & \cmark &  &  &  & \cmark & \cmark &  \\
& GRAND$^\dag$~\cite{feng2020graph} & \cmark &  &  & \cmark &  & \cmark & \\
\cmidrule(lr){2-10}
& MVGRL~\cite{hassani2020contrastive} & \cmark &  &  &  & \cmark &  &  & \multirow{2}{1in}{Graph diffusion} \\
& MV-CGC~\cite{yuan2021semi} & \cmark &  &  &  & \cmark &  &  \\
\cmidrule(lr){2-10}
& JOAO~\cite{you2021graph} &  & \cmark &  & \cmark & \cmark & \cmark & \cmark & \multirow{5}{1in}{Automated augmentation} \\
& GCA~\cite{zhu2021graph} & \cmark &  &  &  & \cmark & \cmark &  \\
& LG2AR~\cite{hassani2022learning} & \cmark &  &  & \cmark & \cmark & \cmark & \cmark \\
& FairAug~\cite{kose2022fair} & \cmark &  &  & \cmark & \cmark & \cmark &  \\
& AD-GCL~\cite{suresh2021adversarial} & \cmark &  &  & \cmark &  &  &  \\
\cmidrule(lr){2-10}
& NodeAug$^\dag$~\cite{wang2020nodeaug} & \cmark &  &  &  & \cmark & \cmark &  & Biased perturbation \\
\bottomrule
\end{tabular}}
\end{table*}



% In this section, we discuss GDA techniques that are used for supervised graph learning. We categorize the GDA techniques by their task levels (node, graph, or edge).



% \noindent\wei{option1: simple and learning-based augmentation}\\
% \wei{option2:  node/edge/feature/subgraph}\\
% \wei{option3: node/edge/graph tasks}
% \wei{option4: }


% \wei{to add adversarial training on graphs}

% \wei{to add imbalanced learning on graphs, e.g., GraphSMOTE}

\subsection{Node-level Tasks}
% \label{sec:sl-node}
% \paragraph{Edge Dropping} Edge dropping methods stochastically remove a certain amount of edges from the graph data during each training epoch. \citet{rong2019dropedge} first proposed DropEdge which randomly dropped a fixed fraction of edges in each epoch, in a way similar to Dropout. By showing the GNN model different part of the graph in each training epoch, DropEdge significantly improved the model's generalization and alleviates the over-smoothing problems of GNNs, especially for deeper GNNs. Although DropEdge efficiently augmented the edges, it is often criticized for also removing task-relevant signals and corrupting informative graph structures.
%such as graph communities. 

% Following DropEdge, \citet{zheng2020robust} proposed NeuralSparse that utilized a MLP-based graph sparsification model that learned to remove only the potentially task-irrelevant edges. The graph sparsification model is supervised and trained jointly with GNN on the node classification loss. PTDNet~\cite{luo2021learning} further applied the nuclear norm regularization loss to impose the low-rank constraint on the modified graph by the graph sparsification model. 
% \citet{luo2021learning} showed the graph sparsification model with the low-rank constraint can effectively prune more task-irrelevant edges from the graph. 
% \citet{gao2021training} proposed TADropEdge that leveraged the graph spectrum to generate edge weights that represent the edges' criticality for the graph connectivity. TADropEdge dropped the edges using the edges weights as the probabilities. 

% Other than node classification, \citet{spinelli2021fairdrop} proposed FairDrop for the task of fair graph representation learning, which biasedly dropped edges with a sensitive attribute homophily mask to protect against unfairness.

% \paragraph{Graph Diffusion} \citet{klicpera2019diffusion} first proposed generalized graph diffusion that modeled a ``future'' state of the graph where the signals were more spread out. By utilizing commonly used graph diffusion such as personalized PageRank (PPR) or heat kernal along with graph sparsification, GDC~\cite{klicpera2019diffusion} generates a diffused version of the observed graph. The generated graph is then used for both training and inferencing. While message passing-based GNNs are only capable of aggregating one hop information in each layer, GDC allows GNNs to learn from multi-hop information without specifically re-designing the model.

% To further utilize the information given by different graph diffusions, MV-GCN~\cite{yuan2021semi} generates two complementary views with PPR and heat kernal and learns from both created views and the original graph. Then the three views of the graph are fed into three GCNs. MV-GCN uses a consistency regularization loss to reduce the distribution distance of the representations learned from the three views. The final node representations for downstream tasks is the combination of the three.

% \paragraph{Structure Prediction}
% Prediction-based GDA techniques update the graph structure to enhance task-relevant information in the graph. For example, \citet{zhao2021data} showed the correlation between graph structural homophily and node classification performance. Then they proposed GAug-M and GAug-O to update the graph structure by neural link predictors. Similar to GDC~\cite{klicpera2019diffusion}, GAug-M deterministically modifies the graph structure and use the updated graph for training and inferencing. To allow inductive learning on graphs, GAug-O samples graph structure from learned probabilities
% from the edge probabilities learned by the link predictor 
% in each training epoch. 
% \citet{chen2020measuring} also proposed AdaEdge that iteratively add/remove edges according to the node classification prediction. In each iteration, after the GNN model is sufficiently trained, AdaEdge adds edges between nodes that are predicted to be in the same class with high confidence, and vice versa. AdaEdge iteratively performs GNN training and graph modification until convergence. 
% Pro-GNN~\cite{jin2020graph} updates the graph structure with constrains on the low-rank property and feature smoothness.

% MH-Aug~\cite{park2021metropolis} creates an ``explicit'' target distribution, with controlled strength and diversity, to sample augmented graphs. As sampling from the complex target distribution is infeasible, MH-Aug adopts the Metropolis-Hastings algorithm to obtain the augmented samples.

% \citet{zhao2021action} proposed Eland for the task of anomaly detection on time-stamped user-item bipartite graphs. Eland first transforms the user-item graph into users' action sequences and adopts seq2seq model for future action prediction. The predicted user actions are added back into the graph to generate the augmented graph data. As the augmented graph contains richer user behavior information, Eland enhances the anomaly detection performance and detects anomalies at an early stage.

% \paragraph{Feature Augmentation}
% For (semi-)supervised graph learning, 
% % instead of randomly masking off the features, 
% feature augmentation methods usually try to improve the node feature quality by learning additional task-relevant features.
% FLAG~\cite{kong2020flag} utilizes adversarial training to iteratively augment the node features with gradient-based adversarial perturbations. Being a free training approach, FLAG improves the performances of GNNs on the tasks of node classification, link prediction, and graph classification.
% LA-GNN~\cite{liu2021local} enhances the locality of node representations by generating additional node features based on the conditional distribution of the local structures and neighbor features. LA-GNN learns the new features of each node by the conditional distribution of its local neighborhood. The generated feature is directly used together with the raw node features. Similarly, SR+DR~\cite{song2021topological} generates topology features with DeepWalk~\cite{perozzi2014deepwalk}, and uses a dual GNN model with topology regularization to jointly train with both raw and topology features.

% \paragraph{Mixup}
% Mixup~\cite{zhang2018mixup} merges two images to generate a new images with a weighted label. 
% Given the dependent and non-Euclidean structure of graph, the direct analog of Mixup on graph data is not obvious. 
% \citet{verma2019graphmix} proposed GraphMix that augmented the training of a GNNs with a Fully-Connected Network, which is trained by interpolating the hidden states and labels. 
% As GraphMix is more of a regularization method than the analog of Mixup on graphs, \citet{wang2021mixup} proposed Graph Mixup, which analogized Mixup with a two-branch graph convolution module. Given a pair of nodes, Graph Mixup mixes the raw features of them, feeds the them into the two-branch GNN layer, and mixes their hidden representations of each layer. Mixing up the nodes on features and hidden states avoids re-assembling the local neighborhoods of the two nodes.

% \paragraph{Pseudo-labeling}
% todo

% \paragraph{AutoML}
% With the rapid development of AutoML, automated graph learning method were proposed to automate the design of GNN architecture as well as the choice of GDA operations. \citet{sun2021automated} proposed AutoGRL for the task of node classification. Though training process, AutoGRL learns the best combination of GDA operations, GNN architecture, and hyperparameters. The searching space of AutoGRL includes four GDA operations implemented by random masking and GAug-M~\cite{zhao2021data}: drop features, drop nodes, add edges, and remove edges.


\subsection{Graph-level Tasks}
\label{sec:sl-graph}
% For graph-level tasks, where data objects are independent graphs, certain augmentation operations in CV and NLP can be transferred to graph data. For example, similar to image cropping, GraphCrop~\cite{wang2020graphcrop} crops a contiguous subgraph from each of the given graph object. GraphCrop adopts a graph diffusion-based node-centric strategy
% % , performing graph diffusion on the randomly selected seed nodes, 
% to maintain the topology characteristics of original graphs. 

% M-Evolve~\cite{zhou2020data} utilizes motifs to augment the graph data. M-Evolve first finds and selects the target motif in the graph, then adds or removes edges within the selected motifs based on a sampling weight calculated with Resource Allocation index.
% Similarly, MoCL~\cite{sun2021mocl} utilizes biomedical domain knowledge to augment the molecular graphs on the substructures such as functional groups. 
% MoCL selects a substructure from each molecular graph and replaces it with another substructure. 

% \paragraph{Mixup} 
% Several Mixup methods were also proposed for graph classification. For example, the aforementioned Graph Mixup~\cite{wang2021mixup} also works for graph classification. 
% % To avoid the node matching problem when mixing up two independent graphs, 
% Graph Mixup mixes the latent representations of the pair of graphs. 
% On the other hand, ifMixup~\cite{guo2021intrusion} directly applies Mixup on the graph data instead of the latent space. As the pair of graphs are irregular and the nodes from two graphs are not aligned, ifMixup arbitrarily assigns indices to the nodes in each graph and matches the nodes according to the indices. 
% Empirically, ifMixup shows marginal performance improvements over Graph Mixup on the task of graph classification.
% Following ifMixup, Graph Transparent~\cite{park2021graph} also mixes graph in data space. Unlike ifMixup that randomly matches nodes during mixing, Graph Transparent uses substructures as mixing units to preserve the local structural information. Graph Transparent employs the node saliency information to select one meaningful substructure from each graph, where the saliency information is defines as the $l_2$ norm of the gradient of the classification loss. \wei{to add G-mixup~\cite{han2022G}; also need to  reflect this change in the table }

% \paragraph{Graph Rationalization}
% TODO

\subsection{Edge-level Tasks}
% \label{sec:sl-edge}
% We note that very few GDA techniques were proposed for edge level tasks such as link prediction. \citet{zhao2021counterfactual} proposed a counterfactual data augmentation method CFLP. CFLP asks the counterfactual question of ``would the link still exist if the graph structure became different from observation?'' To answer the question, \citet{zhao2021counterfactual} proposed counterfactual links that approximates the unobserved outcome in the question. CFLP trains the link prediction model with both the given training data and the generated counterfactual links (as augmented data).

% \citet{wang2021adaptive} proposed MeTA for link prediction on temporal graphs. MeTA contains a multi-level module that processes the augmented graphs of different magnitudes on separate levels. MeTA adopted three augmentation operations for the temporal graphs: perturb time that modifies the time-stamp on edges, remove edge that is similar to DropEdge~\cite{rong2019dropedge}, and add edges that repeats existing edges with a different time-stamp. During training and prediction, MeTA performs message passing across levels to provide adaptively augmented input graphs.


==> 9gda-ssl.tex <==


% In this section, we cover the GDA techniques that are used for self-supervised learning objectives, i.e., contrastive learning and consistency learning. Self-supervised objectives learn representations that are robust to noise and perturbations by maximizing the (dis)agreements of learned representations. Therefore, unlike the above presented GDA techniques that aim to enhance the task-relevant information in the data, most of the GDA techniques for self-supervised learning are stochastic augmentations that aims to corrupt the given graph data. Moreover, most self-supervised graph representation learning methods tend to use a combination of several simple GDA operations.

% \wei{robustness? anomaly detection?}

% \subsection{Contrastive Learning}
% \label{sec:ssl-contrast}
% In the past few years, with the rapid development of contrastive learning, several graph contrastive learning methods~\cite{you2021graph} have been proposed. Contrastive learning aims to maximize the distance between representations of different objects and minimize the distance between representations learned from different views of the same object. Data augmentation is commonly used for generating the different views for contrastive learning. 

% \paragraph{Corruption} 
% vTo efficiently generate different augmented data for graph contrastive learning, the most commonly used GDA operations are the corruption-based ones. For example, DGI~\cite{velickovic2019deep} adopts feature corruption where it conducts a row-wise shuffling on the raw node feature matrix $\mathbf{X}$. The feature corruption by DGI can also be viewed as randomly swapping the nodes in the graph. 

% GraphCL~\cite{you2020graph} and InfoGCL~\cite{xu2021infogcl} adopt four GDA operations: node dropping that randomly removes nodes along with its edges, edge perturbation that randomly adds or drops edges, attribute masking that randomly masks off certain node attributes, and subgraph sampling that samples a connected subgraph. Similar to the subgraph sampling operation used in GraphCL, SUBG-CON~\cite{jiao2020sub} utilizes a subgraph sampler to sample the augmented subgraph.
% GRACE~\cite{zhu2020deep} and BGRL~\cite{thakoor2022largescale} use only the basic random edge dropping and attribute masking for creating different views of the graph. 

% \paragraph{Graph diffusion} 
% As an efficient GDA operation that can naturally creates a ``future view'' of the given graph, graph diffusion is also used in graph contrastive learning. MVGRL~\cite{hassani2020contrastive} adopts the diffusion graph proposed by GDC~\cite{klicpera2019diffusion} as the second view. Interestingly, \citet{hassani2020contrastive} showed that using three views (original graph, diffusion graphs by PPR and heat kernal) would not result with better performance than using two views (original graph and one diffusion graph), and concluded ``increasing the number of views does not improve the performance.'' However, \citet{yuan2021semi} later proposed MV-CGC that adopted a similar contrastive learning framework with three views: original graph, diffusion graph, and their proposed feature similarity view. Empirically, the node representations learned by MV-CGC outperformed those learned by MVGRL on
% % the task of 
% node classification.


% \paragraph{Automated GDA}
% As aforementioned, most contrastive learning methods adopt a combination of several simple augmentation operations. The selection among the operations and their magnitudes significantly increases the number of hyperparameters. Therefore, automated solutions that can learn the augmentation strategies are developed.

% JOAO~\cite{you2021graph} models the selection of GDA for GraphCL~\cite{you2020graph} as a bilevel optimization problem, where the outer level learns the augmentation strategy and the inner level learns graph representations with the given augmentations.
% AD-GCL~\cite{suresh2021adversarial} utilizes an adversarial graph augmentation strategy to avoid redundant information brought by random augmentation.
% LG2AR~\cite{hassani2022learning} learns a probabilistic policy that contains a set of distributions over different augmentation operations, and samples augmentation strategy from the policy in each training epoch.
% GCA~\cite{zhu2021graph} designs adaptive augmentations based on the node centrality measures. Unlike the above-mentioned that finds the best augmentation strategy for the dataset, the adaptive augmentation of GCA gives different augmentation to nodes according to their importance. Similarly, FairAug~\cite{kose2022fair} utilizes adaptive augmentation for fair graph representation learning.


% \subsection{Consistency Learning}
% \label{sec:ssl-consistent}
% Similar to contrastive learning, consistency learning learns representation from different views of data and maximizes their agreement. However, unlike contrastive learning that compares between data objects, the consistency loss compares the distributions of a batch of representations via metrics like KL-divergence. Therefore, the consistency loss is rarely used itself, but often used along with supervised losses in the semi-supervised learning. 
% For example, NodeAug~\cite{wang2020nodeaug} uses three local structure-based augmentation operations: replace attributes, remove edges, and add edges. NodeAug minimizes the KL-divergence between the node representations learned from the original graph and augmented graph. GRAND~\cite{feng2020graph} creates multiple different augmented graphs with node dropping and feature masking. The consistency loss then minimizes the distances of the representations learned from the augmented graphs.







==> ref_gliu.tex <==
%%% update: neurips 2022

%  theoretical analysis for heuristic graph data augmentation (edge/node editing) in self-supervised (contrastive) learning
@article{trivedi2022analyzing,
  title={Analyzing Data-Centric Properties for Contrastive Learning on Graphs},
  author={Trivedi, Puja and Lubana, Ekdeep Singh and Heimann, Mark and Koutra, Danai and Thiagarajan, Jayaraman J},
  journal={arXiv preprint arXiv:2208.02810},
  year={2022}
}
%  theoretical analysis for data augmentation for images
@article{balestriero2022data,
  title={A data-augmentation is worth a thousand samples: Exact quantification from analytical augmented sample moments},
  author={Balestriero, Randall and Misra, Ishan and LeCun, Yann},
  journal={arXiv preprint arXiv:2202.08325},
  year={2022}
}

%  theoretical analysis for the effect data augmentation in classifications
@article{balestriero2022effects,
  title={The effects of regularization and data augmentation are class dependent},
  author={Balestriero, Randall and Bottou, Leon and LeCun, Yann},
  journal={arXiv preprint arXiv:2204.03632},
  year={2022}
}


% Knowledge Distillation Improves Graph Structure Augmentation for Graph Neural Networks. not available yet.

% What Makes a "Good" Data Augmentation in Knowledge Distillation - A Statistical Perspective. not available

% Augmentations in Hypergraph Contrastive Learning: Fabricated and Generative % Tianxin Wei · Yuning You · Tianlong Chen · Yang Shen · Jingrui He · Zhangyang Wang. Not available.

@article{yue2022label,
  title={Label-invariant Augmentation for Semi-Supervised Graph Classification},
  author={Yue, Han and Zhang, Chunhui and Zhang, Chuxu and Liu, Hongfu},
  journal={arXiv preprint arXiv:2205.09802},
  year={2022}
}

%%% update neurips 2022 end







% arxiv. graph-level augmentation in the latent space for graph property classification.
@article{yue2022label,
  title={Label-invariant Augmentation for Semi-Supervised Graph Classification},
  author={Yue, Han and Zhang, Chunhui and Zhang, Chuxu and Liu, Hongfu},
  journal={arXiv preprint arXiv:2205.09802},
  year={2022}
}


@article{liu2021graph,
  title={A graph data augmentation strategy with entropy preserving},
  author={Liu, Xue and Sun, Dan and Wei, Wei},
  journal={arXiv preprint arXiv:2107.06048},
  year={2021}
}


% KDD 22
% (not available) Enhancing Machine Learning Approaches for Graph Optimization Problems with Diversifying Graph Augmentation % Chen-Hsu Yang (National Tsing Hua University); Chih-Ya Shen (National Tsing Hua University)* 


% (not available) Enhancing Machine Learning Approaches for Graph Optimization Problems with Diversifying Graph Augmentation % Chen-Hsu Yang (National Tsing Hua University); Chih-Ya Shen (National Tsing Hua University)*  
% Robust Tensor Graph Convolutional Networks via T-SVD based Graph Augmentation. Zhebin Wu (Sun Yat-Sen University)*; Lin Shu (Sun Yat-sen University); Ziyue Xu (Sun Yat-Sen University); Yaomin Chang (Sun Yat-sen University); Chuan Chen (Sun Yat-sen University); Zibin Zheng (Sun Yat-sen University)


% augment more graphs for a rationale subgraph based on different environment subgraphs
@article{liu2022graph,
  title={Graph Rationalization with Environment-based Augmentations},
  author={Liu, Gang and Zhao, Tong and Xu, Jiaxin and Luo, Tengfei and Jiang, Meng},
  journal={arXiv preprint arXiv:2206.02886},
  year={2022}
}

% augmentations (e.g. edge perturbation) may lead to bias (for node-level tasks). proposed to augment on the hidden features by maintaining a “good sketch” of original features
@article{zhang2022costa,
  title={COSTA: Covariance-Preserving Feature Augmentation for Graph Contrastive Learning},
  author={Zhang, Yifei and Zhu, Hao and Song, Zixing and Koniusz, Piotr and King, Irwin},
  journal={arXiv preprint arXiv:2206.04726},
  year={2022}
}


@article{li2022edge,
  title={Edge Augmentation on Disconnected Graphs via Eigenvalue Elevation},
  author={Li, Tianyi},
  journal={arXiv preprint arXiv:2207.05301},
  year={2022}
}

% ICLR 2022
% augmentations for data(node) imbalance
@inproceedings{park2021graphens,
  title={GraphENS: Neighbor-Aware Ego Network Synthesis for Class-Imbalanced Node Classification},
  author={Park, Joonhyung and Song, Jaeyun and Yang, Eunho},
  booktitle={International Conference on Learning Representations},
  year={2022}
}



%% propose two metrics, Consistency and Diversity, from the aspects of augmentation correctness and generalization. attemp to find a graph augmentation satisfying both consistency and diversity
@article{BoHu2022, 
    title={Regularizing Graph Neural Networks via Consistency-Diversity Graph Augmentations}, volume={36}, 
    DOI={10.1609/aaai.v36i4.20307}, 
    number={4}, 
    journal={Proceedings of the AAAI Conference on Artificial Intelligence}, 
    author={Bo, Deyu and Hu, Binbin and Wang, Xiao and Zhang, Zhiqiang and Shi, Chuan and Zhou, Jun}, year={2022}, 
    month={Jun.}, 
    pages={3913-3921} 
}
%% non-graph
% class-wise augmentation
@article{rommel2021cadda,
  title={CADDA: Class-wise automatic differentiable data augmentation for EEG signals},
  author={Rommel, C{\'e}dric and Moreau, Thomas and Paillard, Joseph and Gramfort, Alexandre},
  journal={arXiv preprint arXiv:2106.13695},
  year={2021}
}
@inproceedings{cheung2021adaaug,
  title={AdaAug: Learning Class-and Instance-adaptive Data Augmentation Policies},
  author={Cheung, Tsz-Him and Yeung, Dit-Yan},
  booktitle={International Conference on Learning Representations},
  year={2022}
}

% The main novelty of NFM against manifold mixup lies in the injection of noise when taking convex combinations of pairs of input and hidden layer features
@inproceedings{lim2021noisy,
  title={Noisy Feature Mixup},
  author={Lim, Soon Hoe and Erichson, N Benjamin and Utrera, Francisco and Xu, Winnie and Mahoney, Michael W},
  booktitle={International Conference on Learning Representations},
  year={2022}
}




